Memorize and Rank: Elevating Large Language Models for Clinical Diagnosis Prediction

Clinical diagnosis prediction models, when provided with a patient's medical history, aim to detect potential diseases early, facilitating timely intervention and improving prognostic outcomes. However, the inherent scarcity of patient data and large disease candidate space often pose challenges in developing satisfactory models for this intricate task. The exploration of leveraging Large Language Models (LLMs) for encapsulating clinical decision processes has been limited. We introduce MERA, a clinical diagnosis prediction model that bridges pertaining natural language knowledge with medical practice. We apply hierarchical contrastive learning on a disease candidate ranking list to alleviate the large decision space issue. With concept memorization through fine-tuning, we bridge the natural language clinical knowledge with medical codes. Experimental results on MIMIC-III and IV datasets show that MERA achieves the state-of-the-art diagnosis prediction performance and dramatically elevates the diagnosis prediction capabilities of generative LMs.

==> content/110_limitation.tex <==
\section{Limitations}
\label{appendix: limitation}
We would like to raise awareness that there might be miscoded diagnosis codes in the patient records. The billing ICD diagnosis codes are used as “ground-truth” diagnosis decisions to train our model and evaluate the performance for diagnosis prediction. We acknowledge that the diagnosis code extracted from the EHR dataset should not be considered the best/perfect diagnosis decision. We also raise the potential data distribution issue as the training and evaluation data used in this work is largely collected for patients with ICU stay history. Thus, the evaluation result does not represent the generalized diagnosis prediction capability, and the trained model may yield compromised performance when different kinds of patient records are queried.

==> content/120_impact.tex <==
\section{Broader Impact Statement}
\label{appendix: impact}
\modelname contributes to the potential improvement of healthcare delivery and patient outcomes. By aiming to accurately predict diseases based on patient medical histories, these models offer a possibility for earlier detection and intervention, which might lead to better patient outcomes over time. Given the challenges associated with limited patient data and the complexity of diagnosing a wide range of diseases, \modelname's approach, which leverages Large Language Models (LLMs) and hierarchical contrastive learning, represents a step towards addressing these issues. While its performance on the MIMIC datasets indicates promising results in diagnosis prediction, the real-world application of such models underscores the cautious optimism for AI's role in enhancing clinical decisions and healthcare efficiency. These developments suggest a direction where AI could support more informed clinical decisions, potentially improving patient care and management, albeit with ongoing evaluation and validation needed to fully realize these benefits.



==> content/130_ethics.tex <==
\section{Ethical Statement}
\label{appendix: ethics}
While \modelname demonstrates improved performance in diagnostic prediction tasks, the trained model may incorporate biases from multiple sources, including the pre-training corpus or the medical records distribution utilized for fine-tuning, and more. Therefore, the model necessitates comprehensive evaluation prior to its consideration for real-world clinical application. Additionally, the outcomes of the diagnostic prediction model may not be utilized to attribute discriminatory labels to specific diseases. Healthcare institutions and insurance entities may not use the predictive diagnoses of \modelname as a basis for changing patient services.

==> table/data_stats.tex <==
\begin{table}[h]
\begin{center}
{
\small
\begin{tabular}{l|rr}
\toprule
Dataset & MIMIC-III & MIMIC-IV 
\\ \midrule
\# unique patients & 7493 & 10000 
\\
Train/valid/test splits & 6000/493/1000 & 8000/1000/1000
\\
Max. \# visit & 42 & 55
\\
Avg. \# visit & 2.66 & 3.66
\\ \hline
\# unique diagnosis codes & 4880 & 6102 
\\
Max. \# codes per visit & 39 & 50
\\
Avg. \# codes per visit & 13.06 & 13.38
\\
\bottomrule
\end{tabular}
}
\end{center}
\caption{
Data statistics.
}
\label{table:data_stats}
\end{table}
